Active MR k-space Sampling with Reinforcement Learning

Deep learning approaches have recently shown great promise in accelerating magnetic resonance image (MRI) acquisition. The majority of existing work have focused on designing better reconstruction models given a pre-determined acquisition trajectory, ignoring the question of trajectory optimization. In this paper, we focus on learning acquisition trajectories given a fixed image reconstruction model. We formulate the problem as a sequential decision process and propose the use of reinforcement learning to solve it. Experiments on a large scale public MRI dataset of knees show that our proposed models significantly outperform the state-of-the-art in active MRI acquisition, over a large range of acceleration factors.

==> 2_related.tex <==
% Active learning for touch~\cite{Yi2016Active}.

%% Acquisition Policies for MRI
% Basic Compressed Sensing (CS) techniques reconstruct MR images from under-sampled k-space measurements \cite{lustig2007comprsensingmri}. It accelerates the acquisition process at the cost of introducing artifacts in the reconstructed image. Data prior based regularization techniques improve the image quality but slow down the reconstruction process. However, efficient optimization techniques \cite{Boyd2011ADMM} coupled with deep architectures for hyper-parameter search \cite{Yang2016DeepAF} lead to fast and accurate CS based MR acquisition processes.

% Various deep learning architectures \cite{Wang2016Accelerating,Schlemper2017DeepCascade,Chen2018Variable,Zhu2018Image,Lonning2019Recurrent,Zhang_2019_CVPR} learn the mapping between MRIs reconstructed from under-sampled and fully sampled k-space to reconstruct higher quality MR images than CS.  But the trained reconstructor networks might not perform well when the training and test data has different Signal to Noise Ratio (SNR), image contrast, sampling pattern etc. Researchers studied the generalization capabilities of the deep reconstruction networks and demonstrated the potential of transfer learning by pre-training the networks with synthetic data and fine-tuning them with a subset of the training set \cite{Knoll2019Assesment}.


Previous acquisition techniques (compressed sensing, deep learning based approaches). See: \cite{Zhang_2019_CVPR,bahadir2019learning,jin2019self,weiss2019learning}


==> 5_methodology.tex <==
\md{This part seems to be too general. Can we ground this section a bit more in our problem or move it to background? Alternatively, it might be enough to cite DQN and DDQN and shorten the description...}


\iffalse
% Currently, the standard approach for learning in sequential decision problems is the use of deep reinforcement learning (DRL) ~\cite{mnih2013playing,lillicrap2015continuous,mnih2016asynchronous,schulman2017proximal,hessel2018rainbow,haarnoja2018soft}. 
Considering that our problem involves discrete actions, we have opted for the deep Q-network (\textsc{dqn}) algorithm~\cite{mnih2013playing}, and, specifically, its more robust \textsc{double-dqn} variant~\cite{van2016deep}, which we denote as \textsc{ddqn}. In \textsc{dqn} and \textsc{ddqn}, a neural network is used to approximate the \emph{utility} of each action, and a policy $\pi$ can be recovered by choosing actions greedily with respect to this utility. We start our description focusing on \textsc{dqn}, and explain the extension to \textsc{ddqn} below.

\textsc{dqn} requires the specification of a \emph{value network}, which provides estimates of the utility of each action for a given observation. The value network has an output for each possible available action, representing the expected utility of taking the action at that state and following an optimal policy afterwards. In the RL literature, this utility is referred to as a \emph{Q-value}~\cite{sutton2018reinforcement}, and must satisfy the following \emph{Bellman equation}:
\[
    Q(\mathbf{s}_t, a_t; \theta) = \mathbb{E}_{\mathbf{s}_{t+1}\sim \mathcal{E}} \big[ R(\mathbf{s}_t, a_t) + \gamma \max_{a'} Q(\mathbf{s}_{t+1}, a'; \theta)\big],
\]
where $\mathcal{E}$ represents the environment, $\gamma$ is a discount factor, and $\theta$ represents the model parameters. Following the Q-learning algorithm~\cite{watkins1992q} for Q-value estimation, in \textsc{dqn} the value network is trained to minimize the temporal difference error~\cite{sutton1988learning}:

\[
\mathcal{TD}(\theta) = \mathbb{E}_{\mathbf{s}_t, a_t\sim \rho} \big[ (z - Q(\mathbf{s}_t, a_t; \theta)^2\big], 
\]
where $\rho$ is a \emph{replay memory} of states and actions acquired through an exploration policy, and $z$ is a target defined for \textsc{ddqn} as: 
\[z \triangleq \mathbb{E}_{\mathbf{s}_{t+1}\sim \mathcal{E}} \big[ R(\mathbf{s}_t, a) + \gamma Q\big(\mathbf{s}_{t+1}, \argmax_{a'} Q(\mathbf{s}_t, a'; \theta); \theta'\big)\big].
\]
Note that to increase training stability, this target uses a separate \emph{target network} parametrized by $\theta'$ that is updated periodically: $\theta' \leftarrow \theta$. Further stability is obtained by performing the $\arg\max$ operator with the \emph{online network} (parameters $\theta$), as shown in the equation; more details can be found in the \textsc{ddqn} paper~\cite{van2016deep}. %The \textsc{ddqn} variant follows the formulation above almost exactly, with the only exception that the the $\argmax$ is taken with respect to $Q(\cdot, a; \theta)$ rather than the target network; this has been shown to further stabilize training~\cite{van2016deep}. 
Finally, once the $Q$-network has been trained, a policy can be recovered by choosing the action with highest $Q$-value for each observation, $\mathbf{s}_t$.
\fi

For our value network, we used the neural architecture proposed by~\cite{Zhang_2019_CVPR}, which receives as input a reconstructed image, $\hat{\mathbf{x}_t}$, and a mask $\mathbf{M}_t$. %While the architecture is shared between the two methods, they are in fact trained very differently. 
Note that the model proposed by~\cite{Zhang_2019_CVPR} myopically chooses the $k$-space column that has the highest estimated impact in reconstruction MSE, with respect to the ground truth image. In contrast, our \textsc{dqn} model is trained to produce a sequence of $k$-space columns that maximizes the reconstruction quality over a full range of MRI acquisition \emph{trajectories}. As mentioned in Section~\ref{sec:problem_form}, the acquisition system is not allowed to choose repeated actions. 
%Therefore, we take the $\max$ in the target only over all valid actions for the current state. 
In practice, we manually set $Q(\mathbf{s}_t, a') \leftarrow -\infty$ whenever $\mathbf{M}_t(.,a')=\mathbf{1}$. Additionally, for the exploration policy, we use a modified $\epsilon$-greedy policy~\cite{sutton2018reinforcement}, which chooses the best action with probability $1-\epsilon$, and with probability $\epsilon$ chooses an action from the set of valid actions. \md{The last sentence is unclear to me, there is no mention about exploration previously in the manuscript.}

Finally, although the description of \textsc{dqn} above focuses on the MDP case, the same approach can be used to solve POMDPs, with few modifications. For the POMDP case, policies are functions of observation-action histories, rather than individual states (which are now hidden). This is typically handled via auto-regressive models~\cite{hausknecht2015deep,hochreiter1997long} that receive observation $\mathbf{o}_t$ as inputs. In our work we opt for only passing the last observation (i.e., reconstruction) as input, since the mask and the reconstruction essentially summarize all the history of observations. It's possible that using recurrence would improve performance, but exploring this alternative is left as future work.

%Alternatively, optimal policies can be computed as a function of \emph{belief states}~\cite{kaelbling1998planning}, which are probability distributions over the set of possible states. %; in fact, every POMDP is equivalent to an MDP whose states are the beliefs of the original problem. 
% In our case, since we can essentially obtain belief states from our probabilistic reconstructor (see Section~\ref{sec:background}), we opt for a standard \textsc{dqn} approach that receives the output of the reconstructor as its sole input. In particular, for our experiments we use the mean reconstruction estimate as input to the \textsc{dqn} model, ignoring uncertainty information.\footnote{In the POMDP planning literature, this is sometimes referred to as the \emph{most-likely-state} heuristic.}~While it is possible that including this information in the model input would improve its performance, we leave this direction for future work. 

% We learn the acquisition policy on a set of training images using function approximation.


% The POMDP defined in the previous section is very high-dimensional, and thus impractical to solve using exact and optimal algorithms \luis{add citation}. To address this issue, we opt for a data-driven approach, in which an active acquisition policy is learned on a set of training images using function approximation; the learned policy can then be subsequently used to perform efficient inference at test time. The current standard framework for learning in sequential decision problems is the use of deep reinforcement learning (DRL). 

% \subsection{Deep Q-networks}

% There are many DRL algorithms for solving MDPs and POMDPs~\cite{mnih2013playing,lillicrap2015continuous,mnih2016asynchronous,schulman2017proximal,hessel2018rainbow,haarnoja2018soft}. Considering that our problem involves discrete actions, we have opted for the deep Q-network (\textsc{dqn}) algorithm~\cite{mnih2013playing}, and, specifically, its more robust \textsc{double-dqn} variant~\cite{van2016deep}. \textsc{dqn} has seen widespread usage on a variety of scenarios and it is easy to implement and tune. While more advanced algorithms are now available, we argue that it is a natural first choice to study the applicability of DRL for active MRI acquisition.

% MD: I do not find this necesary at this point. If we really want to keep this discussion, I'd move it to the problem formulation section.
% \subsection{Using DQN for solving POMDPs}

% In general, optimal policies for POMDPs are functions of observation-action histories, rather than of individual observations. In the DRL literature, this is typically handled by using auto-regressive models~\cite{hausknecht2015deep,hochreiter1997long}, or by using multiple observation as inputs~\cite{mnih2013playing}. Alternatively, optimal policies can be computed as a function of \emph{belief states}~\cite{kaelbling1998planning}, which are probability distributions over the set of possible states; in fact, every POMDP is equivalent to an MDP whose states are the beliefs of the original problem. In our case, since we can essentially obtain belief states from our probabilistic reconstructor (see Section~\ref{sec:background}), we opt for a standard \textsc{dqn} approach that receives the output of the reconstructor as its sole input. In particular, for our experiments we use the mean reconstruction estimate as input to the \textsc{dqn} model, ignoring uncertainty information.\footnote{In the POMDP planning literature, this is sometimes referred to as the \emph{most-likely-state} heuristic.}~While it is possible that including this information in the model input would improve its performance, we leave this direction for future work. 
 
